Scalable and Efficient Continual Learning from Demonstration via a Hypernetwork-generated Stable Dynamics Model

Robots capable of learning from demonstration (LfD) must exhibit stability while executing learned motion skills. To be effective in the real world, they should also remember multiple skills over time -- a capability lacking in current stable-LfD methods. We propose an approach to stable, continual LfD, and highlight the role of stability in improving continual learning. Our proposed hypernetwork generates the parameters of two neural networks: a trajectory learning dynamics model, and a trajectory-stabilizing Lyapunov function. These generated networks form a clock-augmented stable neural ODE solver (sNODE), a stable dynamics model that offers a superior stability-accuracy trade-off compared to the state-of-the-art. We further propose stochastic hypernetwork regularization with a single, uniformly-sampled task embedding, reducing the cumulative training time for $N$ tasks from O($N^2$) to O($N$) without degrading performance on real-world tasks. We introduce high-dimensional variants of the popular LASA dataset to assess scalability and extend a dataset of robotic LfD tasks to assess real-world performance. We empirically evaluate our approach on multiple LfD datasets of varying complexity, including sequences of 7--26 tasks, trajectories of 2--32 dimensions, and real-world tasks involving position and orientation. Our thorough evaluation on multiple LfD datasets demonstrates that our approach sequentially learns and retains multiple motion skills without retraining on past demonstrations, and outperforms other relevant baselines in terms of trajectory errors, continual learning scores, and stability metrics. Notably, we show that stability greatly enhances continual learning performance, particularly in size-efficient chunked hypernetworks. Our code is available at https://github.com/sayantanauddy/clfd-snode.

==> figures/LASA_highD_all_lsddm.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
MET & ACC & REM & MS & TE & FS & SSS & CL$_{sco}$ & CL$_{stab}$ \\
\midrule
SG & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 1.00 & 0.29 & \cellcolor{white} \bfseries 1.00 & 0.00 & \cellcolor{white} \bfseries 1.00 & 0.71 & 0.55 \\
FT & 0.18 & 0.02 & 1.00 & 0.99 & \cellcolor{white} \bfseries 0.87 & \cellcolor{white} \bfseries 1.00 & 0.68 & 0.55 \\
REP & 0.77 & \cellcolor{white} \bfseries 1.00 & 1.00 & 0.99 & \cellcolor{white} \bfseries 0.87 & 0.45 & 0.85 & 0.78 \\
HN & 0.97 & 1.00 & \cellcolor{white} \bfseries 1.00 & 0.85 & 0.64 & \cellcolor{white} \bfseries 1.00 & 0.91 & 0.85 \\
CHN & 0.86 & 1.00 & 1.00 & 0.81 & 0.84 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 0.92 & \cellcolor{white} \bfseries 0.90 \\
\bottomrule
\end{tabular}


==> figures/LASA_highD_all_node.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
MET & ACC & REM & MS & TE & FS & SSS & CL$_{sco}$ & CL$_{stab}$ \\
\midrule
SG & \cellcolor{white} \bfseries 0.99 & \cellcolor{white} \bfseries 1.00 & 0.29 & \cellcolor{white} \bfseries 1.00 & 0.00 & \cellcolor{white} \bfseries 1.00 & 0.71 & 0.55 \\
FT & 0.18 & 0.02 & 1.00 & 0.99 & \cellcolor{white} \bfseries 0.89 & \cellcolor{white} \bfseries 1.00 & 0.68 & 0.55 \\
REP & 0.74 & 0.99 & 1.00 & 0.99 & \cellcolor{white} \bfseries 0.89 & 0.45 & 0.85 & 0.78 \\
HN & 0.92 & 0.99 & \cellcolor{white} \bfseries 1.00 & 0.64 & 0.65 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 0.87 & \cellcolor{white} \bfseries 0.82 \\
CHN & 0.72 & 0.99 & 1.00 & 0.60 & 0.86 & \cellcolor{white} \bfseries 1.00 & 0.86 & 0.82 \\
\bottomrule
\end{tabular}


==> figures/rt9_posoricombined_lsddm.tex <==
\begin{tabular}{rrrrrrrr}
\toprule
ACC & REM & MS & TE & FS & SSS & CL$_{sco}$ & CL$_{stab}$ \\
\midrule
\cellcolor{white} \bfseries 0.92 & \cellcolor{white} \bfseries 1.00 & 0.31 & \cellcolor{white} \bfseries 0.99 & 0.00 & \cellcolor{white} \bfseries 1.00 & 0.70 & 0.56 \\
0.19 & 0.05 & 1.00 & 0.98 & \cellcolor{white} \bfseries 0.86 & \cellcolor{white} \bfseries 1.00 & 0.68 & 0.56 \\
0.86 & 1.00 & 1.00 & 0.98 & \cellcolor{white} \bfseries 0.86 & 0.44 & 0.86 & 0.79 \\
0.89 & 0.99 & \cellcolor{white} \bfseries 1.00 & 0.86 & 0.44 & \cellcolor{white} \bfseries 1.00 & 0.86 & 0.78 \\
0.79 & 0.98 & 1.00 & 0.87 & 0.84 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 0.91 & \cellcolor{white} \bfseries 0.91 \\
\bottomrule
\end{tabular}


==> figures/rt9_posoricombined_node.tex <==
\begin{tabular}{rrrrrrrr}
\toprule
ACC & REM & MS & TE & FS & SSS & CL$_{sco}$ & CL$_{stab}$ \\
\midrule
\cellcolor{white} \bfseries 0.89 & \cellcolor{white} \bfseries 1.00 & 0.31 & \cellcolor{white} \bfseries 1.00 & 0.00 & \cellcolor{white} \bfseries 1.00 & 0.70 & 0.57 \\
0.17 & 0.15 & 1.00 & 1.00 & \cellcolor{white} \bfseries 0.87 & \cellcolor{white} \bfseries 1.00 & 0.70 & 0.58 \\
0.67 & 0.96 & 1.00 & 0.99 & \cellcolor{white} \bfseries 0.87 & 0.44 & 0.82 & 0.77 \\
0.77 & 1.00 & \cellcolor{white} \bfseries 1.00 & 0.68 & 0.54 & \cellcolor{white} \bfseries 1.00 & 0.83 & 0.80 \\
0.61 & 0.92 & 1.00 & 0.70 & 0.84 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 0.85 & \cellcolor{white} \bfseries 0.84 \\
\bottomrule
\end{tabular}


==> figures/tables_lasa16d_node_cl.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
MET & ACC & REM & MS & TE & FS & SSS & CL$_{sco}$ & CL$_{stab}$ \\
\midrule
SG & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 1.00 & 0.29 & \cellcolor{white} \bfseries 1.00 & 0.00 & \cellcolor{white} \bfseries 1.00 & 0.72 & 0.55 \\
FT & 0.18 & 0.00 & 1.00 & 1.00 & \cellcolor{white} \bfseries 0.89 & \cellcolor{white} \bfseries 1.00 & 0.68 & 0.54 \\
REP & 0.82 & \cellcolor{white} \bfseries 1.00 & 1.00 & 0.99 & \cellcolor{white} \bfseries 0.89 & 0.45 & 0.86 & 0.79 \\
HN & 0.93 & 0.99 & \cellcolor{white} \bfseries 1.00 & 0.64 & 0.62 & \cellcolor{white} \bfseries 1.00 & 0.86 & 0.82 \\
CHN & 0.82 & \cellcolor{white} \bfseries 1.00 & 1.00 & 0.59 & 0.87 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 0.88 & \cellcolor{white} \bfseries 0.84 \\
\bottomrule
\end{tabular}


==> figures/tables_lasa16d_snode_cl.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
MET & ACC & REM & MS & TE & FS & SSS & CL$_{sco}$ & CL$_{stab}$ \\
\midrule
SG & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 1.00 & 0.29 & \cellcolor{white} \bfseries 0.99 & 0.00 & \cellcolor{white} \bfseries 1.00 & 0.71 & 0.55 \\
FT & 0.18 & 0.00 & 1.00 & 0.99 & \cellcolor{white} \bfseries 0.89 & \cellcolor{white} \bfseries 1.00 & 0.68 & 0.54 \\
REP & 0.80 & \cellcolor{white} \bfseries 1.00 & 1.00 & 0.99 & \cellcolor{white} \bfseries 0.89 & 0.45 & 0.85 & 0.79 \\
HN & 0.99 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 1.00 & 0.84 & 0.70 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 0.92 & 0.88 \\
CHN & 0.85 & 1.00 & 1.00 & 0.82 & 0.87 & \cellcolor{white} \bfseries 1.00 & \bfseries 0.92 & \cellcolor{white} \bfseries 0.91 \\
\bottomrule
\end{tabular}


==> figures/tables_lasa2d_node_cl.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
MET & ACC & REM & MS & TE & FS & SSS & CL$_{sco}$ & CL$_{stab}$ \\
\midrule
SG & \cellcolor{white} \bfseries 0.89 & \cellcolor{white} \bfseries 1.00 & 0.15 & 0.99 & 0.00 & \cellcolor{white} \bfseries 1.00 & 0.67 & 0.53 \\
FT & 0.06 & 0.19 & 1.00 & \cellcolor{white} \bfseries 0.99 & 0.96 & \cellcolor{white} \bfseries 1.00 & 0.70 & 0.55 \\
REP & 0.56 & \cellcolor{white} \bfseries 1.00 & 1.00 & 0.99 & 0.96 & 0.48 & 0.83 & 0.76 \\
SI & 0.05 & 0.36 & \cellcolor{white} \bfseries 1.00 & 0.92 & 0.78 & \cellcolor{white} \bfseries 1.00 & 0.68 & 0.61 \\
MAS & 0.01 & 0.87 & 1.00 & 0.89 & 0.83 & \cellcolor{white} \bfseries 1.00 & 0.76 & 0.62 \\
HN & 0.80 & 0.96 & 1.00 & 0.46 & 0.90 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 0.85 & \cellcolor{white} \bfseries 0.79 \\
CHN & 0.39 & 0.72 & 1.00 & 0.45 & \cellcolor{white} \bfseries 0.96 & \cellcolor{white} \bfseries 1.00 & 0.75 & 0.72 \\
\bottomrule
\end{tabular}


==> figures/tables_lasa2d_snode_cl.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
MET & ACC & REM & MS & TE & FS & SSS & CL$_{sco}$ & CL$_{stab}$ \\
\midrule
SG & 0.87 & \cellcolor{white} \bfseries 1.00 & 0.15 & 0.99 & 0.00 & \cellcolor{white} \bfseries 1.00 & 0.67 & 0.54 \\
FT & 0.06 & 0.20 & 1.00 & 0.98 & 0.95 & \cellcolor{white} \bfseries 1.00 & 0.70 & 0.56 \\
REP & 0.73 & \cellcolor{white} \bfseries 1.00 & 1.00 & \cellcolor{white} \bfseries 0.99 & 0.95 & 0.48 & 0.86 & 0.79 \\
SI & 0.02 & 0.53 & \cellcolor{white} \bfseries 1.00 & 0.97 & 0.75 & \cellcolor{white} \bfseries 1.00 & 0.71 & 0.62 \\
MAS & 0.08 & 0.38 & 1.00 & 0.86 & 0.80 & \cellcolor{white} \bfseries 1.00 & 0.69 & 0.63 \\
HN & \cellcolor{white} \bfseries 0.88 & 0.98 & 1.00 & 0.71 & 0.88 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 0.91 & \cellcolor{white} \bfseries 0.89 \\
CHN & 0.70 & 0.90 & 1.00 & 0.71 & \cellcolor{white} \bfseries 0.96 & \cellcolor{white} \bfseries 1.00 & 0.88 & 0.86 \\
\bottomrule
\end{tabular}


==> figures/tables_lasa32d_node_cl.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
MET & ACC & REM & MS & TE & FS & SSS & CL$_{sco}$ & CL$_{stab}$ \\
\midrule
SG & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 1.00 & 0.29 & \cellcolor{white} \bfseries 1.00 & 0.00 & \cellcolor{white} \bfseries 1.00 & 0.71 & 0.55 \\
FT & 0.18 & 0.00 & 1.00 & 0.98 & \cellcolor{white} \bfseries 0.89 & \cellcolor{white} \bfseries 1.00 & 0.68 & 0.54 \\
REP & 0.85 & \cellcolor{white} \bfseries 1.00 & 1.00 & 0.99 & \cellcolor{white} \bfseries 0.89 & 0.45 & 0.86 & 0.79 \\
HN & 0.99 & 1.00 & \cellcolor{white} \bfseries 1.00 & 0.64 & 0.72 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 0.89 & \cellcolor{white} \bfseries 0.83 \\
CHN & 0.82 & 0.99 & 1.00 & 0.57 & 0.87 & \cellcolor{white} \bfseries 1.00 & 0.88 & \bfseries 0.83 \\
\bottomrule
\end{tabular}


==> figures/tables_lasa32d_snode_cl.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
MET & ACC & REM & MS & TE & FS & SSS & CL$_{sco}$ & CL$_{stab}$ \\
\midrule
SG & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 1.00 & 0.29 & \cellcolor{white} \bfseries 1.00 & 0.00 & \cellcolor{white} \bfseries 1.00 & 0.72 & 0.55 \\
FT & 0.18 & 0.01 & 1.00 & 0.99 & \cellcolor{white} \bfseries 0.88 & \cellcolor{white} \bfseries 1.00 & 0.68 & 0.55 \\
REP & 0.84 & \cellcolor{white} \bfseries 1.00 & 1.00 & 0.99 & \cellcolor{white} \bfseries 0.88 & 0.45 & 0.86 & 0.79 \\
HN & 0.99 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 1.00 & 0.84 & 0.72 & \cellcolor{white} \bfseries 1.00 & 0.92 & 0.88 \\
CHN & 0.93 & 1.00 & 1.00 & 0.77 & 0.87 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 0.93 & \cellcolor{white} \bfseries 0.91 \\
\bottomrule
\end{tabular}


==> figures/tables_lasa8d_node_cl.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
MET & ACC & REM & MS & TE & FS & SSS & CL$_{sco}$ & CL$_{stab}$ \\
\midrule
SG & \cellcolor{white} \bfseries 0.96 & \cellcolor{white} \bfseries 1.00 & 0.29 & 1.00 & 0.00 & \cellcolor{white} \bfseries 1.00 & 0.71 & 0.55 \\
FT & 0.18 & 0.06 & 1.00 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 0.89 & \cellcolor{white} \bfseries 1.00 & 0.69 & 0.56 \\
REP & 0.56 & 0.98 & 1.00 & 1.00 & \cellcolor{white} \bfseries 0.89 & 0.45 & 0.81 & 0.76 \\
HN & 0.83 & 0.99 & \cellcolor{white} \bfseries 1.00 & 0.64 & 0.62 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 0.85 & \cellcolor{white} \bfseries 0.82 \\
CHN & 0.52 & 0.98 & 1.00 & 0.65 & 0.82 & \cellcolor{white} \bfseries 1.00 & 0.83 & 0.80 \\
\bottomrule
\end{tabular}


==> figures/tables_lasa8d_snode_cl.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
MET & ACC & REM & MS & TE & FS & SSS & CL$_{sco}$ & CL$_{stab}$ \\
\midrule
SG & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 1.00 & 0.29 & \cellcolor{white} \bfseries 1.00 & 0.00 & \cellcolor{white} \bfseries 1.00 & 0.72 & 0.55 \\
FT & 0.18 & 0.04 & 1.00 & 0.99 & \cellcolor{white} \bfseries 0.84 & \cellcolor{white} \bfseries 1.00 & 0.68 & 0.55 \\
REP & 0.69 & \cellcolor{white} \bfseries 1.00 & 1.00 & 0.99 & \cellcolor{white} \bfseries 0.84 & 0.45 & 0.83 & 0.78 \\
HN & 0.94 & 0.99 & \cellcolor{white} \bfseries 1.00 & 0.87 & 0.49 & \cellcolor{white} \bfseries 1.00 & 0.88 & 0.80 \\
CHN & 0.79 & 0.99 & 1.00 & 0.84 & 0.77 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 0.90 & \cellcolor{white} \bfseries 0.89 \\
\bottomrule
\end{tabular}


==> figures/tables_robottaskspositionorientation6d_node_ori_cl.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
MET & ACC & REM & MS & TE & FS & SSS & CL$_{sco}$ & CL$_{stab}$ \\
\midrule
SG & \cellcolor{white} \bfseries 0.90 & \cellcolor{white} \bfseries 1.00 & 0.31 & \cellcolor{white} \bfseries 1.00 & 0.00 & \cellcolor{white} \bfseries 1.00 & 0.70 & 0.56 \\
FT & 0.17 & 0.14 & 1.00 & 1.00 & \cellcolor{white} \bfseries 0.87 & \cellcolor{white} \bfseries 1.00 & 0.70 & 0.58 \\
REP & 0.74 & 0.97 & 1.00 & 0.99 & \cellcolor{white} \bfseries 0.87 & 0.44 & 0.84 & 0.78 \\
HN & 0.78 & 1.00 & \cellcolor{white} \bfseries 1.00 & 0.68 & 0.54 & \cellcolor{white} \bfseries 1.00 & 0.83 & 0.80 \\
CHN & 0.69 & 0.90 & 1.00 & 0.70 & 0.84 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 0.86 & \cellcolor{white} \bfseries 0.86 \\
\bottomrule
\end{tabular}


==> figures/tables_robottaskspositionorientation6d_node_pos_cl.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
MET & ACC & REM & MS & TE & FS & SSS & CL$_{sco}$ & CL$_{stab}$ \\
\midrule
SG & \cellcolor{white} \bfseries 0.87 & \cellcolor{white} \bfseries 1.00 & 0.31 & \cellcolor{white} \bfseries 1.00 & 0.00 & \cellcolor{white} \bfseries 1.00 & 0.70 & 0.57 \\
FT & 0.16 & 0.16 & 1.00 & 1.00 & \cellcolor{white} \bfseries 0.87 & \cellcolor{white} \bfseries 1.00 & 0.70 & 0.58 \\
REP & 0.60 & 0.96 & 1.00 & 0.99 & \cellcolor{white} \bfseries 0.87 & 0.44 & 0.81 & 0.77 \\
HN & 0.76 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 1.00 & 0.68 & 0.54 & \cellcolor{white} \bfseries 1.00 & 0.83 & 0.80 \\
CHN & 0.53 & 0.95 & 1.00 & 0.70 & 0.84 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 0.84 & \cellcolor{white} \bfseries 0.81 \\
\bottomrule
\end{tabular}


==> figures/tables_robottaskspositionorientation6d_snode_ori_cl.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
MET & ACC & REM & MS & TE & FS & SSS & CL$_{sco}$ & CL$_{stab}$ \\
\midrule
SG & \cellcolor{white} \bfseries 0.96 & \cellcolor{white} \bfseries 1.00 & 0.31 & \cellcolor{white} \bfseries 0.99 & 0.00 & \cellcolor{white} \bfseries 1.00 & 0.71 & 0.56 \\
FT & 0.20 & 0.01 & 1.00 & 0.98 & \cellcolor{white} \bfseries 0.86 & \cellcolor{white} \bfseries 1.00 & 0.67 & 0.55 \\
REP & 0.92 & 1.00 & 1.00 & 0.98 & \cellcolor{white} \bfseries 0.86 & 0.44 & 0.87 & 0.79 \\
HN & 0.92 & 0.99 & \cellcolor{white} \bfseries 1.00 & 0.86 & 0.44 & \cellcolor{white} \bfseries 1.00 & 0.87 & 0.78 \\
CHN & 0.86 & 0.98 & 1.00 & 0.87 & 0.84 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 0.92 & \cellcolor{white} \bfseries 0.92 \\
\bottomrule
\end{tabular}


==> figures/tables_robottaskspositionorientation6d_snode_pos_cl.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
MET & ACC & REM & MS & TE & FS & SSS & CL$_{sco}$ & CL$_{stab}$ \\
\midrule
SG & \cellcolor{white} \bfseries 0.88 & \cellcolor{white} \bfseries 1.00 & 0.31 & \cellcolor{white} \bfseries 0.99 & 0.00 & \cellcolor{white} \bfseries 1.00 & 0.70 & 0.57 \\
FT & 0.17 & 0.08 & 1.00 & 0.98 & \cellcolor{white} \bfseries 0.86 & \cellcolor{white} \bfseries 1.00 & 0.68 & 0.57 \\
REP & 0.80 & \cellcolor{white} \bfseries 1.00 & 1.00 & 0.98 & \cellcolor{white} \bfseries 0.86 & 0.44 & 0.85 & 0.79 \\
HN & 0.85 & 0.99 & \cellcolor{white} \bfseries 1.00 & 0.86 & 0.44 & \cellcolor{white} \bfseries 1.00 & 0.86 & 0.78 \\
CHN & 0.73 & 0.97 & 1.00 & 0.87 & 0.84 & \cellcolor{white} \bfseries 1.00 & \cellcolor{white} \bfseries 0.90 & \cellcolor{white} \bfseries 0.89 \\
\bottomrule
\end{tabular}

